The tidal deformation and atmosphere of WASP-12b from its phase curve

Ultra-hot Jupiters present a unique opportunity to understand the physics and chemistry of planets at extreme conditions. WASP-12b stands out as an archetype of this class of exoplanets. We performed comprehensive analyses of the transits, occultations, and phase curves of WASP-12b by combining new CHEOPS observations with previous TESS and Spitzer data to measure the planet's tidal deformation, atmospheric properties, and orbital decay rate. The planet was modeled as a triaxial ellipsoid parameterized by the second-order fluid Love number, $h_2$, which quantifies its radial deformation and provides insight into the interior structure. We measured the tidal deformation of WASP-12b and estimated a Love number of $h_2=1.55_{-0.49}^{+0.45}$ (at 3.2$\sigma$) from its phase curve. We measured occultation depths of $333\pm24$ppm and $493\pm29$ppm in the CHEOPS and TESS bands, respectively, while the dayside emission spectrum indicates that CHEOPS and TESS probe similar pressure levels in the atmosphere at a temperature of 2900K. We also estimated low geometric albedos of $0.086\pm0.017$ and $0.01\pm0.023$ in the CHEOPS and TESS passbands, respectively, suggesting the absence of reflective clouds in the dayside of the WASP-12b. The CHEOPS occultations do not show strong evidence for variability in the dayside atmosphere of the planet. Finally, we refine the orbital decay rate by 12% to a value of -30.23$\pm$0.82 ms/yr. WASP-12b becomes the second exoplanet, after WASP-103b, for which the Love number has been measured (at 3$sigma$) from the effect of tidal deformation in the light curve. However, constraining the core mass fraction of the planet requires measuring $h_2$ with a higher precision. This can be achieved with high signal-to-noise observations with JWST since the phase curve amplitude, and consequently the induced tidal deformation effect, is higher in the infrared.

==> tables/def_fit_result.tex <==

\begin{table}[!t]
\caption{Derived parameters of \plname from the ellipsoidal planet and spherical planet model fits to the datasets.}
\label{tab:def_fit_result}
\centering
\begin{tabular}{ll|ll}
\hline\hline
Parameter     & Prior      & \begin{tabular}[c]{@{}c@{}}Ellipsoidal Model\\fit (E)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Spherical Model\\fit (S)\end{tabular} \\ \hline
$b$              & $\mathcal{U}$(0, 1)         & $0.365\pm0.017$           & $0.391\pm0.014$ \\
$a\,[R_{\star}]$ & $\mathcal{U}$(2.5, 3.5)     & $3.039\pm0.02$            & $3.003\pm0.017$\\
$\log Q_m$       & $\mathcal{N}$(-6.935, 0.025)& $-6.938\pm{0.022}$        & – \\
\hf              & $\mathcal{U}$(0, 2.5)       & $1.553_{-0.518}^{+0.460}$ & –\\[0.8em]

\begin{tabular}[c]{@{}l@{}}\Rv/$R_{\star_{_{\mathrm{CHEOPS}}}}$\\
\Rv/$R_{\star_{_{\mathrm{TESS}}}}$\\
\Rv/$R_{\star_{_{\mathrm{Spitzer3.6}}}}$\\
\Rv/$R_{\star_{_{\mathrm{Spitzer4.5}}}}$\\\end{tabular} &\begin{tabular}[c]{@{}l@{}}$\mathcal{U}$(0, 0.25)\\ $\,$\\ $\,$\\ $\,$\\\end{tabular} &
\begin{tabular}[c]{@{}l@{}} $0.1247\pm0.0023$  \\$0.1224\pm0.0022$ \\$0.1180\pm0.0018$\\ $0.1130\pm0.0017$\end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $0.1180\pm0.0002$\\   $0.1163\pm0.0002$\\$0.1124\pm0.0004$\\  $0.1083\pm0.0006$\end{tabular}\\[2em]

\begin{tabular}[c]{@{}l@{}}$c_{_{\mathrm{CHEOPS}}}$\\ $\alpha_{_{\mathrm{CHEOPS}}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$\mathcal{N}$(0.712, 0.010)\\ $\mathcal{N}$(0.632, 0.022)\end{tabular} & 
    \begin{tabular}[c]{@{}l@{}}$0.715\pm0.006$\\ $0.628\pm0.010$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.718\pm{0.0064}$\\ $0.620\pm{0.010}$\end{tabular} \\[0.8em]
  
\begin{tabular}[c]{@{}l@{}}$c_{_{\mathrm{TESS}}}$\\ $\alpha_{_{\mathrm{TESS}}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$\mathcal{N}$(0.636, 0.012)\\ $\mathcal{N}$(0.554, 0.021)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.638\pm0.007$\\$0.552\pm0.011$ \end{tabular}  &
  \begin{tabular}[c]{@{}l@{}}$0.636\pm0.007$\\$0.545\pm0.010$ \end{tabular}\\[0.8em]

\begin{tabular}[c]{@{}l@{}}$c_{_{\mathrm{Spitzer3.6}}}$\\ $\alpha_{_{\mathrm{Spitzer3.6}}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$\mathcal{N}$(0.313, 0.011)\\ $\mathcal{N}$(0.351, 0.015)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.316\pm0.008$\\$0.348\pm0.011$ \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.317\pm0.010$\\$0.346\pm0.011$ \end{tabular} \\[0.8em]

\begin{tabular}[c]{@{}l@{}}$c_{_{\,\mathrm{Spitzer4.5}}}$\\ $\alpha_{_{\mathrm{Spitzer4.5}}}$\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$\mathcal{N}$(0.245, 0.011)\\ $\mathcal{N}$(0.398, 0.022)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.241\pm0.010$\\$0.406\pm0.020$ \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}$0.240\pm0.096$\\$0.406\pm0.019$ \end{tabular} \\[0.8em]
  Derived\\
  \hline
\begin{tabular}[c]{@{}l@{}}\Rv\,[$R_{\mathrm{Jup}}]_{_{\mathrm{CHEOPS}}}$\\
\Rv\,[$R_{\mathrm{Jup}}]\,_{_{\mathrm{TESS}}}$\\
\Rv\,[$R_{\mathrm{Jup}}]\,_{_{\mathrm{Spitzer3.6}}}$\\
\Rv\,[$R_{\mathrm{Jup}}]\,_{_{\mathrm{Spitzer4.5}}}$\\\end{tabular} &\begin{tabular}[c]{@{}l@{}} \\ $\,$\\ $\,$\\ $\,$\\\end{tabular} &
\begin{tabular}[c]{@{}l@{}} $2.102\pm0.044$  \\$2.066\pm0.043$ \\$1.991\pm0.040$\\ $1.907\pm0.038$\end{tabular}  &
\begin{tabular}[c]{@{}l@{}} $1.992\pm0.025$\\   $1.961\pm0.025$\\$1.897\pm0.025$\\  $1.828\pm0.025$\end{tabular}\\[2em]

  

  \hline
\end{tabular}
\end{table}

